Anisotropic Microgels show their Soft Side

Anisotropic, submicrometer sized particles are versatile systems providing interesting features in creating ordering in 2-dimensional systems. Combining hard ellipsoids with a soft shell further enhances the opportunities to trigger and control order and alignment. In this work, we report a rich 2D phase behavior and show how softness affects the ordering of anisotropic particles at fluid oil-water interfaces. Three different core-shell systems were synthesized such that they have the same elliptical hematite-silica core but differ with respect to thickness and stiffness of the soft microgel shell. Compression isotherms, the shape of individual core-shell microgel as well as their 2D order at a decane-water interface are investigated by means of the Langmuir-Blodgett technique combined with ex-situ Atomic Force Microscopy (AFM) imaging, as well as by Disspiative Particle Dynamics (DPD) simulations. We show how softness, size and anisotropy of the microgel shell affect the side-to-side vs. tip-to-tip ordering of anisotropic hybrid microgels as well as the alignment with respect to the direction of compression in the Langmuir trough. A large and soft microgel shell leads to an ordered structure with a tip-to-tip alignment directed perpendicular to the direction of compression. In contrast, a thin and harder microgel shell leads to side-to-side ordering orientated parallel to the compression direction. In addition, the thin and harder microgel shell induces clustering of the microgels in the dilute state indicating the presence of strong capillary interactions. Our findings highlight the relevance of softness for the complex ordering of anisotropic hybrid microgels at interfaces.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
